Category-Specific Object Reconstruction from a Single Image

Object reconstruction from a single image -- in the wild -- is a problem where we can make progress and get meaningful results today. This is the main message of this paper, which introduces an automated pipeline with pixels as inputs and 3D surfaces of various rigid categories as outputs in images of realistic scenes. At the core of our approach are deformable 3D models that can be learned from 2D annotations available in existing object detection datasets, that can be driven by noisy automatic object segmentations and which we complement with a bottom-up module for recovering high-frequency shape details. We perform a comprehensive quantitative analysis and ablation study of our approach using the recently introduced PASCAL 3D+ dataset and show very encouraging automatic reconstructions on PASCAL VOC.

==> DenseModels.tex <==
\label{densemodels}
Equipped with camera projection parameters and keypoint correspondences (now lifted to 3D by \nrsfm) on the whole training set, we proceed to build morphable 3D models for object categories from our major source of information in this paper - object silhouettes. This problem of reconstructing the 3D shape of a single object from its projected silhouettes in multiple calibrated images has been widely studied in the computer vision literature. Two prominent approaches are \textit{visual hulls} \cite{laurentini1994hull} and variational methods derived from \textit{snakes} e.g \cite{esteban2004snake,yusuf2006snake} which deform a surface mesh iteratively until convergence. Some recent papers have also extended variational approaches to the case of category shape reconstruction \cite{cashman2013dolphins,chen20123d}. While demonstrating accurate results on a limited number of categories, they typically require some form of 3D annotations to bootstrap the model and are computationally expensive. A recent work \cite{carvi14} has proposed a visual-hull based data-driven approach for class-based reconstruction for the first time on challenging real world datasets like PASCAL VOC. In contrast, we build parametric shape models for categories that compactly capture intra class shape variations. The benefits of having a model of 3D shape are manifold: 1) we are more robust to noisy inputs (silhouettes and pose) allowing us to pursue reconstruction in a fully automatic setting and 2) we forego the need for having continuous access to a large corpus of data. \RED{add points here.}

We propose an algorithm to learn class-specific 3D shape models given silhouette information and camera viewpoints estimated in the previous section. Our shape models inherently capture the intraclass variations in object categories and can be used to recover a 3D shape given an object's approximate silhouette and viewpoint in a new image.


==> VisualHullModels.tex <==
\subsection{Prototype Shape Models}
\label{VH}

Parametric models with simple deformations might not sufficiently capture large intra-class variance which is frequently present in some categories. Allowing complex deformations, on the other hand, would result in a significant increase in the computational complexity as well as the possibility of overfitting. We explore whether representing category shapes via multiple learned prototypes can alleviate these issues. We propose to learn a representative set of 3D prototypes for a category employing variations of visual hull techniques that we make more robust to intra-class variation and noisy camera estimates.

A key observation which enables this approach is that an estimate of a coarse rotation invariant shape parameter allows grouping of visually similar instances into ``visual clusters". Deriving our prototypes from these visual clusters provides an effective way of modeling the various modes of the distribution underlying the shapes of an object category. Formally, we infer our shape model from a training set $T:\{(O^i,P^i,\alpha^i)\}$, where the quantities $O_i$ and $P_i$ are as described in the previous section. The additional input $\alpha^i$ corresponds to the coarse rotation invariant shape parameter which in our implementation is the deformation weight vector obtained using the NRSfM algorithm. Note that the proposed approach can exploit any coarse shape parameter (e.g. simple cues based on the silhouette shape).

\subsubsection{Learning:}
\begin{figure}[htb!]
\centering
\begin{minipage}{.45\textwidth}

  \includegraphics[width=.45\linewidth]{figures/visClusters1.jpg}
  \label{fig:VisCluster1}
\quad
%\begin{subfigure}{.22\textwidth}
  \includegraphics[width=.45\linewidth]{figures/visClustersShape1.jpg}
  \label{fig:VisShape1}
%\end{subfigure}

%\begin{subfigure}{.22\textwidth}
  \includegraphics[width=.45\linewidth]{figures/visClusters2.jpg}
  \label{fig:VisCluster2}
%\end{subfigure}%
\quad
%\begin{subfigure}{.22\textwidth}
  \includegraphics[width=.45\linewidth]{figures/visClustersShape2.jpg}
  \label{fig:VisShape2}
%\end{subfigure}
\vspace{7pt}
  
\caption{Learned prototype shapes corresponding to different visual clusters.}
\label{fig:visClusterShapes}
\end{minipage}
\hspace{0.05\textwidth}
%\vspace*{\fill}
%\begin{center}
\begin{minipage}{.45\textwidth}

\centering
 \includegraphics[width = \linewidth]{figures/visHullPlanes.jpg}
%\vspace{-5}
\caption{Illustration of visual cones induced by silhouettes.}
\label{fig:visHullPlanes}

\end{minipage}
%\end{center}

%\vfill
\end{figure}


%\begin{figure}[htb!]
%\centering
% \includegraphics[scale = 0.2]{figures/visHullPlanes.jpg}
%\caption{Illustration of visual cones induced by silhouettes.}
%\label{fig:visHullPlanes}
%\end{figure}

We represent the shape model $M = \{ (\bar{S_k},\alpha_k) | k=1..K\}$ as a set of volumetric shape representations $\bar{S_k}$ and associated shape parameters $\alpha_k$. The individual prototype $\bar{S_k}$ is learned from the corresponding visual cluster and the associated shape parameter $\alpha_k$ represents the mean deformation parameter for the corresponding cluster.

In fig.~\ref{fig:visClusterShapes}, we visualize some training instances and their ``visual cones" - a visual cone is the volume that projects inside the silhouette under the corresponding orthographic transformation. The visual hull approach for learning a shape model is to take the intersection of all the visual cones and the object volume is then represented as a binary value associated with each voxel. We use an extensible representation based on the truncated signed distance function (TSDF) which is a field over voxel space such that a level set describes the object surface. A TSDF represents the signed distances of points from a surface and the distances are truncated at some minimum and maximum thresholds. We denote a TSDF $S$ whose values are restricted between $[l,L]$ as $S[l,L]$. Thus the prototype $\bar{S_k}$ visual hull from the associated visual cluster $C_k$ is simply
\begin{equation}
\label{eq:VisLearning}
\bar{S_k} = \underset{i \in C_k}{\sum}S^i[0,\infty]
\end{equation}
where $S_i[0,\infty]$ is the TSDF representing the distances from the surface of the visual cone for  $O^i$ under transformation $P^i$. We prefer the TSDF representation because it can be easily extended to handle variations and noise as we describe later. Fig.~\ref{fig:visHullPlanes} shows some visual clusters and the corresponding prototype models that we learn.

\subsubsection{Inference:}
Given an instance $I = (O,P,\alpha)$, we hypothesize that its dense shape would be similar to the shape of the instances in the most similar visual cluster in our model $M = \{ (\bar{S_k},\alpha_k)\}$. Thus, we find its closest cluster $C_j$ in the training set and combine the shape information obtained using the silhouette for the particular instance with the prototype model of $C_j$. We first compute the TSDF $S[0,\infty]$ for the particular instance using $(O,P)$. This volumetric representation is then updated according to equation \ref{eq:inferenceVis} to infer the dense shape for the given instance.
\begin{equation}
\label{eq:inferenceVis}
S \leftarrow S + \lambda \bar{S_j}
\end{equation}
\subsubsection{Allowing for Intra-class Variations and Camera Estimation Error:}
The approach described above learns the visual hull for each visual cluster. However, this may not be the desirable as our camera estimates are not perfect and a visual cluster does not exactly correspond to an instance. We suggest two modifications to make our method more robust -
\begin{itemize}
\item Instead of using a minimum truncation value 0 for the TSDF computations, we allow a small negative value. This results in learned/inferred shapes which differ from the visual hull approach by allowing us to retain the voxels which are consistent with a majority of the instances and violate very few constraints, presumably due to shape variations or noisy camera estimates.
\item The distribution of views for an object class is often non-uniform and to account for this, we modify the learning in equation \ref{eq:VisLearning} to assign an importance weight to each instance. Since we aim to negate the viewpoint bias using these weights, we first cluster the camera viewpoints within each visual cluster. The weight for each instance is then assigned to be inversely proportional to the size of its corresponding viewpoint cluster to normalize for the view distribution.
\end{itemize}


==> overview.tex <==
We adopt a coarse-to-fine approach to reconstruction and build dense shape models progressively. We assume the availability of a small set of consistent per-class keypoint correspondences as well as ground-truth segmentations and take advantage of both to jointly estimate camera viewpoint and rough modes of shape variation within a category. We build upon the Non-rigid Structure-from-Motion (NRSFM) algorithm of Torresani \etal \cite{Torresani2008NRSFM} which can deal with missing data (occluded keypoints) and propose a modification that allows it to leverage object segmentations for improved robustness -- this is described in the next section. Given the viewpoint estimates and deformation weights from NRSFM, our method proceeds to build class shape models much denser than the initial small set of keypoints. We propose two alternative shape models that are obtained using techniques inspired by standard multiview shape-from-silhouette approaches: a dense parametric 3D morphable model (sec. \ref{OPTIMIZ}) and a non-parametric visual hull based model (sec. \ref{VH}). Equipped with these models we can reconstruct a new object given just its keypoints and silhouette, but this results in a dominantly top-down, memory-induced 3D shape which may not align well with the fine shape details that only become apparent when looking at pixels. This motivates our aim to combine top-down with bottom-up reconstruction.

We propose a simple sequential architecture, and render a dense depth map using our top-down shape model, which serves as guidance to a state-of-the-art intrinsic image decomposition algorithm that produces our final outputs: pixelwise object surface depth, normals, albedo and illumination information. Our motivation is that shape-from-shading algorithms are more naturally competent at predicting high frequency localized shape (say bezels and lights in cars), which vary considerably between different object instances, but have trouble capturing rough global shape, which is more stable across a class and that is characterized by long-range dependencies: it seems necessary to reason over different class instances to reliably capture such low-frequency shape information. 

\subsubsection{Intrinsic Images:}We use the SIRFS algorithm of Barron and Malik \cite{barronPAMI13,Barron2012B} which is driven by priors on shape, albedo and illumination that try to capture the statistical regularities in the natural world. For example, shapes are smooth and some colors are more frequent than others. Formally, the SIRFS formulation is:

\begin{equation*}
\begin{aligned}
& \underset{Z,L}{\text{minimize}}
& & g(I-S(Z,L))+f(Z)+h(L)
\end{aligned}
\end{equation*}
where $R=I-S(Z,L)$ is a log-reflectance image, $Z$ is a depth map and $L$ is a spherical-harmonic model of illumination. $S(Z,L)$ is a rendering engine which linearizes $Z$ into a set of surface normals and produces a log shading image with the illumination $L$. $g$, $f$ and $h$ are the loss functions corresponding to reflectance, shape and illumination respectively. 

We use an extended version of SIRFS that allows incorporating a noisy shape observation into the optimization. The loss term corresponding to this is as follows:

\begin{equation*}
f_o(Z,Z') = \underset{i}{\sum}((Z_i-Z_i')^2+\epsilon^2)^{\gamma_o}
\end{equation*}
where $Z'$ is the noisy shape and $\epsilon$ us added to make the loss differentiable everywhere. We use the depth maps obtained from our shape-from-silhouette methods as $Z'$ to better guide the solution to this highly non-convex problem. 


==> resultsFig.tex <==
\begin{figure*}[htb!]
  \includegraphics[width = \textwidth]{figures/reconstructions/1}
  
%  \includegraphics[width = \textwidth]{figures/reconstructions/2}

%   \includegraphics[width = \textwidth]{figures/reconstructions/4} 
 
 \includegraphics[width = \textwidth]{figures/reconstructions/5}    
 
% \includegraphics[width = \textwidth]{figures/reconstructions/28}
 
\includegraphics[width = \textwidth]{figures/reconstructions/29}

 \includegraphics[width = \textwidth]{figures/reconstructions/7}
  
% \includegraphics[width = \textwidth]{figures/reconstructions/8}

   \includegraphics[width = \textwidth]{figures/reconstructions/10}
  
% \includegraphics[width = \textwidth]{figures/reconstructions/11}

 %  \includegraphics[width = \textwidth]{figures/reconstructions/13}
  
 \includegraphics[width = \textwidth]{figures/reconstructions/14}
 \includegraphics[width = \textwidth]{figures/reconstructions/16}
       
%\includegraphics[width = \textwidth]{figures/reconstructions/17}
%\end{figure}
%\begin{figure}
%\includegraphics[width = \textwidth]{figures/reconstructions/19}

\includegraphics[width = \textwidth]{figures/reconstructions/20}

%\includegraphics[width = \textwidth]{figures/reconstructions/22}

\includegraphics[width = \textwidth]{figures/reconstructions/23}

\includegraphics[width = \textwidth]{figures/reconstructions/25}

%\includegraphics[width = \textwidth]{figures/reconstructions/26}

\caption{\label{fig:recons}Example reconstructions of objects shown on the left column. Columns 3 and 4 show the 3D reconstruction obtained using our basis shape model and columns 6 and 7 show the one obtained using our prototype shape model. Columns 2 and 5 show the corresponding final depth maps combining both top-down and bottom-up cues. Blue is closer to the camera, red is farther away.}
\end{figure*}
